Prototype Guided Backdoor Defense

Deep learning models are susceptible to {\em backdoor attacks} involving malicious attackers perturbing a small subset of training data with a {\em trigger} to causes misclassifications. Various triggers have been used, including semantic triggers that are easily realizable without requiring the attacker to manipulate the image. The emergence of generative AI has eased the generation of varied poisoned samples. Robustness across types of triggers is crucial to effective defense. We propose Prototype Guided Backdoor Defense (PGBD), a robust post-hoc defense that scales across different trigger types, including previously unsolved semantic triggers. PGBD exploits displacements in the geometric spaces of activations to penalize movements toward the trigger. This is done using a novel sanitization loss of a post-hoc fine-tuning step. The geometric approach scales easily to all types of attacks. PGBD achieves better performance across all settings. We also present the first defense against a new semantic attack on celebrity face images. Project page: \hyperlink{https://venkatadithya9.github.io/pgbd.github.io/}{this https URL}.

==> sections/Supple/agg_cav_results_backup.tex <==
\begin{table*}[t]
\caption{Results of aggregate PAV configuration on CIFAR10 compared to other configurations}
\label{tab:aggres}
\small
\begin{tabular}
{@{}L{14mm}||C{6.5mm}C{6.5mm}||C{6.5mm}C{6.5mm}|C{6.5mm}C{6.5mm}|C{6.5mm}C{6.5mm}|C{6.5mm}C{6.5mm}||C{6.5mm}C{6.5mm}|C{6.5mm}C{6.5mm}|C{6.5mm}C{6.5mm}|C{6.5mm}C{6.5mm}@{}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \toprule[1.2pt]
\toprule[1.5pt]
% \hline
% Method  & \multicolumn{2}{c||}{Baseline} & \multicolumn{8}{c||}{Ours $T_{pro}$}     & \multicolumn{8}{c}{Ours $T_{syn}$}     \\
METHOD \faCaretRight & \multicolumn{2}{c||}{Baseline} & \multicolumn{4}{c|}{PGBD ($V^p) \quad \delta=0$} & \multicolumn{4}{c||}{PGBD ($V^p) \quad \delta=0.75$}  & \multicolumn{4}{c|}{PGBD ($V^s) \quad \delta=0$} & \multicolumn{4}{c}{PGBD ($V^s) \quad \delta=0.75$}     \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%\hline
\hline
Agg\_PAV \faCaretRight &
  \multicolumn{2}{c||}{$\mathbf{-}$} &
  \multicolumn{2}{c|}{no agg} &
  \multicolumn{2}{c|}{agg} &
    \multicolumn{2}{c|}{no agg} &
  \multicolumn{2}{c||}{agg} &
    \multicolumn{2}{c|}{no agg} &
  \multicolumn{2}{c|}{agg} &
    \multicolumn{2}{c|}{no agg} &
  \multicolumn{2}{c}{agg} \\
% Agg\_PAV \faCaretRight &
%   \multicolumn{1}{c}{$\mathbf{-}$} &
%   \multicolumn{1}{c||}{$\mathbf{-}$} &
%   \multicolumn{1}{c}{no agg} &
%   \multicolumn{1}{c}{no agg} &
%   \multicolumn{1}{c}{agg} &
%   \multicolumn{1}{c|}{agg} &
%   \multicolumn{1}{c}{no agg} &
%   \multicolumn{1}{c}{no agg} &
%   \multicolumn{1}{c}{agg} &
%   \multicolumn{1}{c||}{agg} &
%   \multicolumn{1}{c}{no agg} &
%   \multicolumn{1}{c}{no agg} &
%   \multicolumn{1}{c}{agg} &
%   \multicolumn{1}{c|}{agg} &
%   \multicolumn{1}{c}{no agg} &
%   \multicolumn{1}{c}{no agg} &
%   \multicolumn{1}{c}{agg} &
%   \multicolumn{1}{c}{agg} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule[0.5pt]
%\midrule
ATTACK \faCaretDown & CA  & ASR  & CA & ASR & CA & ASR & CA & ASR & CA & ASR & CA & ASR & CA & ASR & CA & ASR & CA & ASR \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule[1.5pt]
%\specialrule{1.5pt}{1\jot}{1\jot}
% BadNet  &              &               &    &     &    &     &    &     &    &     &    &     &    &     &    &     &    &     \\
% Trojan  &              &               &    &     &    &     &    &     &    &     &    &     &    &     &    &     &    &     \\
% Blended &              &               &    &     &    &     &    &     &    &     &    &     &    &     &    &     &    &     \\
% Signal  &              &               &    &     &    &     &    &     &    &     &    &     &    &     &    &     &    &     \\
% Wanet   &              &               &    &     &    &     &    &     &    &     &    &     &    &     &    &     &    &  \\
Badnet & 92.34 & 88.93 & 92.11 & 0.533 & 88.69 & 0.47 & 90.66 & 0.82 & 88.00 & 0.48 &  92.6 & 0.09 & 89.03 & 10.86 & 91.22 & 1.70 & 89.80 & 0.71 \\ 
Trojan & 93.00 & 100.0 & 92.17 & 90.86 & 87.20 & 74.98 & 83.60 & 6.76 & 86.22 & 37.03 & 92.18 & 99.95 & 90.34 & 4.30 & 76.34 & 2.68 & 87.18 & 17.16 \\ 
Blended & 93.06 & 92.94 & 91.33 & 5.267 & 87.23 & 4.69 & 86.11 & 4.87 & 85.44 & 12.90 & 92.27 & 74.92 & 88.58 & 39.46 & 87.51 & 2.58 & 88.10 & 25.60 \\ 
Sig & 92.90 & 89.04 & 90.72 & 0.19 & 87.13 & 2.12 & 87.18 & 0.31 & 85.80 & 0.24 & 91.58 & 71.08 & 88.10 & 3.64 & 89.94 & 7.51 & 88.93 & 0.29 \\ 
Wanet & 89.98 & 97.60 & 88.81 & 85.35 & 89.47 & 72.10 & 88.54 & 2.36 & 87.67 & 22.14 & 90.72 & 77.28 & 90.77 & 85.37 & 83.61 & 0.61 & 88.70 & 13.08 \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hline
\bottomrule[1.5pt]
\end{tabular}
\end{table*}


% \begin{table*}[]
% \caption{Results of aggregate cav configuration on CIFAR10 compared to other configurations}
% \begin{tabular}{@{}lllllllllllllllllll@{}}
% Attack &
%   \multicolumn{2}{l}{Baseline} &
%   \multicolumn{2}{l}{Ours (\( T_{proto}, \delta = 0\))} &
%   \multicolumn{2}{l}{Ours (\( T_{proto_{agg}}, \delta = 0\))} &
%   Ours (\( T_{proto}, \delta = 0.75\)) &
%    &
%   \multicolumn{2}{l}{Ours (\( T_{proto_{agg}}, \delta = 0.75\))} &
%   \multicolumn{2}{l}{Ours (\( T_{synth}, \delta = 0\))} &
%   \multicolumn{2}{l}{Ours (\( T_{synth_{agg}}, \delta = 0\))} &
%   Ours (\( T_{synth}, \delta = 0.75\)) &
%    &
%   \multicolumn{2}{l}{Ours (\( T_{synth_{agg}}, \delta = 0.75\))} \\
%         & CA & ASR & CA & ASR & CA & ASR & CA & ASR & CA & ASR & CA & ASR & CA & ASR & CA & ASR & CA & ASR  \\
% Badnet  & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -    \\
% Trojan  & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & - \\
% Blended & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -    \\
% Sig     & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -    \\
% Wanet   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   & -  & -   
% \end{tabular}
% \label{tab: agg_cav_results}
% \end{table*}


==> sections/figures/tsne.tex <==
    

==> sections/tables/abl_distill.tex <==
\begin{table*}[tb]
\footnotesize
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{tabular}{l||cc||ccc|ccc||ccc|ccc}
%\begin{tabular}{@{}L{12mm}||C{8mm}C{8mm}||C{8mm}C{8mm}C{8mm}|C{8mm}C{8mm}C{8mm}||C{8mm}C{8mm}C{8mm}|C{8mm}C{8mm}C{8mm}@{}}
\centering
\begin{tabular}{l||cc||ccc|ccc||ccc|ccc}
\toprule[1.2pt]
%\toprule[1pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Method \faCaretRight & \multicolumn{2}{c||}{Baseline} & \multicolumn{6}{c||}{PGBD ($V^p$)} & \multicolumn{6}{c}{PGBD ($V^S$)}\\
%\midrule
%Distill \faCaretRight & \multicolumn{2}{c||}{$-$} & \multicolumn{3}{c|}{\CheckmarkBold} & \multicolumn{3}{c||}{\XSolidBrush} & \multicolumn{3}{c|}{\CheckmarkBold} & \multicolumn{3}{c}{\XSolidBrush} \\
% & & & \multicolumn{3}{c|}{PGBD ($V^p$)} With Distillation} & \multicolumn{3}{c||}{PGBD ($V^p$)} Without Distillation} & \multicolumn{3}{c|}{PGBD ($V^S$) With Distillation} & \multicolumn{3}{c}{PGBD ($V^S$) Without Distillation} \\
Method \faCaretRight & \multicolumn{2}{c||}{Baseline} & \multicolumn{3}{c|}{PGBD($V^p$) with Distil.} & \multicolumn{3}{c||}{PGBD($V^p$) w/o Distil.} & \multicolumn{3}{c|}{PGBD($V^S$) with Distil.} & \multicolumn{3}{c}{PGBD($V^S$) w/o Distil.} \\
%\midrule
Attack \faCaretDown & CA & ASR & CA & ASR & $\Gamma$ & CA & ASR & $\Gamma$ & CA & ASR & $\Gamma$ & CA & ASR & $\Gamma$  \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline %\specialrule{0.75pt}{1\jot}{1\jot}
%\hrule\hrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Badnet  & 92.35 & 88.93  & 90.66  & 0.82 & 0.99 & 73.18 & 0.34 & 0.89 & 91.22  & 1.70 & 0.98 & 82.89 & 0.60 & 0.95 \\
Trojan  & 93.00 & 100.0 & 83.60 & 6.76 & 0.92 & 73.34 & 6.70 & 0.86 & 76.34 & 2.68 & 0.90 & 83.56 & 0.10 & 0.95 \\
Blended & 93.06 & 92.94 & 86.11 & 4.87 & 0.94 & 81.57 & 0.08 & 0.94 & 87.51 & 2.58 & 0.96 & 75.29 & 0.02 & 0.90 \\
Signal  & 92.90 & 89.04 & 87.18 & 0.31 & 0.97 & 71.64 & 0.48 & 0.88 & 89.94 & 7.51 & 0.94 & 82.14 & 0.02 & 0.94 \\
Wanet & 89.98 & 97.60 & 88.54 & 2.36 & 0.98 & 86.90 & 0.09 & 0.98 & 83.61 & 0.61 & 0.96 & 81.10 & 0.01 & 0.95 \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\bottomrule[1pt]
\bottomrule[1.2pt]
\end{tabular}
\caption{Effect of distillation on PGBD ($V^p$) and ($V^s$). Distillation improves performance in all cases except ($V^s$) on Trojan. \TODO{Should we remove $V^S$ from this table and move it to appendix?}}
%\TODO{How do we want to use bold and underline over here. Saurabh sir, would color highlighting be a better option in this case?}}
\label{tab:abl_distill}
\end{table*}


==> sections/tables/abl_no_target.tex <==
\begin{table*}[h!]
\label{tab:abl_no_target}
\caption{Results for the \textit{no target} PGBD on CIFAR10 dataset over 5 attacks}
\centering
    \begin{tabular}{@{}L{20mm}||C{10mm}C{10mm}||C{10mm}C{10mm}C{10mm}|C{10mm}C{10mm}C{10mm}@{}}
    \toprule[1.5pt]
    METHOD \faCaretRight & \multicolumn{2}{c||}{Baseline}   & \multicolumn{3}{c|}{PGBD ($V^p$)} & \multicolumn{3}{c}{PGBD ($V^{p}$) \textit{no target}} \\
    \midrule[0.5pt]
    TARGET \faCaretDown & CA $\uparrow$ & ASR $\downarrow$ & CA $\uparrow$ & ASR $\downarrow$ & $\Gamma \uparrow$ & CA $\uparrow$ & ASR $\downarrow$ & $\Gamma \uparrow$ \\
    \midrule[1.5pt]
    Badnet  & 92.34 & 88.93 & 87.44 & 0.11 & 0.97 & 89.44 & 1.6   & 0.98 \\
    Blended & 93    & 92.9  & 87.41 & 0.76 & 0.97 & 83.48 & 13.3  & 0.88 \\
    Trojan  & 93    & 100   & 89.38 & 3.12 & 0.96 & 73.2  & 19.54 & 0.80 \\
    Signal  & 92.9  & 89.04 & 90.06 & 0.02 & 0.98 & 84.01 & 0.49  & 0.95 \\
    Wanet   & 89.98 & 97.58 & 88.64 & 2.06 & 0.98 & 90.65 & 0.26  & 1.00 \\
    \bottomrule[1.2pt]
    \end{tabular}
\end{table*}

==> sections/tables/abl_pratio.tex <==
% \begin{table}[]
% \caption{Results on varying the poison rate of the train dataset for the Badnet attack with CIFAR10 dataset}
% \begin{tabular}{|l|ll|ll|}
% \hline
% poison ratio & \multicolumn{2}{l|}{Baseline} & \multicolumn{2}{l|}{Ours} \\ \cline{2-5} 
%              & CA            & ASR           & CA          & ASR         \\ \hline
% 0.01         & 92.35         & 88.93         &             &             \\ \hline
% 0.05         & 89.54         & 92.6          &             &             \\ \hline
% 0.1          & 91.57         & 94.85         &             &             \\ \hline
% 0.15         & 90.76         & 96.37         &             &             \\ \hline
% 0.2          & 89.89         & 96.79         &             &             \\ \hline
% \end{tabular}
% \end{table}

\begin{table}[t ]
\centering
\caption{Results on varying the poison ratio of the train dataset for the Badnet attack with CIFAR10 dataset}
\label{tab:abl_pratio}
\small

\begin{tabular}{@{}l||cc||cc@{}}
\toprule[1.2pt]
\toprule[1pt]
METHOD \faCaretRight & \multicolumn{2}{c|}{Baseline}   & \multicolumn{2}{c}{Ours (\(T_{pro}\))} \\
\midrule
POISON RATIO \faCaretDown & CA $\uparrow$ & ASR $\downarrow$ & CA $\uparrow$ & ASR $\downarrow$ \\
\midrule[1pt]
0.01         & 92.35         & 88.93         & 90.66       & 0.82        \\ \hline
0.05         & 90.86         & 96.7          & 92.62       & 0.13        \\ \hline
0.1          & 89.11         & 95.56         & 90.62       & 0.39        \\ \hline
0.15         & 87.69         & 97.88         & 89.72       & 0.17        \\ \hline
0.2          & 85.34         & 98.2          & 90.27       & 0.27        \\ 
\bottomrule[1pt]
\bottomrule[1.2pt]
\end{tabular}
\label{tab:semantic_res}
\end{table}

==> sections/tables/mainRes.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\TODO{Add updated tinyImagenet results to the table}

\begin{table*}[t]
\caption{Quantitative comparison between four different defenses (Finetuning, NAD, I-BAU, MCL) and two of our PGBD variants ($V^p$, $V^s$) for three benchmarks (CIFAR10, CIFAR100, GTSRB). We report three metrics (CA $\uparrow$, ASR $\downarrow$ and $\Gamma \uparrow$) for each of the five attacks types (Badnet, Trojan, Blended, Signal and Wanet). Best and second best values are in \textbf{bold} and \underline{underline} respectively.}
% \small
\footnotesize
\centering
% \begin{tabular}{@{}l||l||cc||ccc|ccc|ccc|ccc||ccc|ccc@{}}
\begin{tabular}{@{}c|l||C{6mm}C{6mm}||C{6mm}C{6mm}C{6mm}|C{6mm}C{6mm}C{6mm}|C{6mm}C{6mm}C{6mm}|C{6mm}C{6mm}C{6mm}||C{6mm}C{6mm}C{6mm}|C{6mm}C{6mm}C{6mm}@{}}
% HEADER
\toprule[1.2pt]
%\toprule[1pt]
% \toprule[1.5pt]
% \multicolumn{1}{c}{} &
  \multicolumn{2}{c||}{Method \faCaretRight} &
  \multicolumn{2}{c||}{Baseline} &
  \multicolumn{3}{c|}{FT} &
  \multicolumn{3}{c|}{NAD} &
  \multicolumn{3}{c|}{I-BAU} &
  \multicolumn{3}{c||}{MCL} &
  \multicolumn{3}{c|}{PGBD ($V^p$)} &
  \multicolumn{3}{c}{PGBD ($V^s$)} \\
\midrule[1.5pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CIFAR 10
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{6}{*}{\STAB{\rotatebox[origin=c]{90}{CIFAR10}}} &
  Attack & CA  & ASR  & CA  & ASR  & $\Gamma$ & CA  & ASR  &  $\Gamma$ & CA  & ASR  & $\Gamma$ & CA  &  ASR & $\Gamma$ & CA  & ASR  & $\Gamma$ & CA  & ASR  & $\Gamma$ \\
\midrule[0.5pt]
& Badnet & 92.34 & 88.93 & 92.66 & 8.43 & 0.95 & 92.64 & 4.92 & 0.97 & 89.56 & 1.81 & 0.97 & 89.76 & 0.01 & \textbf{0.99} & 90.66 & 0.82 & \textbf{0.99} & 91.22 & 1.70 & \underline{0.98} \\
 & Trojan & 93.00 & 100.0 & 93.30 & 99.92 & 0.50 & 93.07 & 99.76 & 0.50 & 63.85 & 10.42 & 0.79 & 78.43 & 8.51 & 0.88 & 83.60 & 6.76 & \textbf{0.92} & 76.34 & 2.68 & \underline{0.90} \\
 & Blended & 93.06 & 92.94 & 93.47 & 92.40 & 0.50 & 80.79 & 3.84 & 0.91 & 81.54 & 2.31 & 0.93 & 90.28 & 2.18 & \textbf{0.97} & 86.11 & 4.87 & 0.94 & 87.51 & 2.58 & \underline{0.96} \\
 & Signal & 92.90 & 89.04 & 93.51 & 83.87 & 0.53 & 81.79 & 6.81 & 0.90 & 89.23 & 18.03 & 0.88 & 80.71 & 4.51 & 0.91 & 87.18 & 0.31 & \textbf{0.97} & 89.94 & 7.51 & \underline{0.94} \\
 & Wanet & 89.98 & 97.60 & 93.39 & 18.37 & 0.91 & 93.32 & 10.87 & 0.94 & 90.90 & 1.30 & \textbf{0.99} & 86.08 & 3.64 & 0.96 & 88.54 & 2.36 & \underline{0.98} & 83.61 & 0.61 & 0.96 \\
\midrule[1.5pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CIFAR 100
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{6}{*}{\STAB{\rotatebox[origin=c]{90}{CIFAR100}}} &
Attack & CA  & ASR  & CA  & ASR  & $\Gamma$ & CA  & ASR  &  $\Gamma$ & CA  & ASR  & $\Gamma$ & CA  &  ASR & $\Gamma$ & CA  & ASR  & $\Gamma$ & CA  & ASR  & $\Gamma$ \\
\midrule[0.5pt]
 & Badnet & 67.32 & 86.98 & 66.82 & 0.43 & \textbf{0.99} & 66.72 & 0.01 & 1.00 & 61.20 & 0.07 & 0.95 & 47.65 & 0.00 & 0.85 & 63.29 & 0.01 & \underline{0.97} & 62.80 & 0.03 & \underline{0.97} \\
 & Trojan & 70.02 & 100.0 & 68.93 & 99.40 & 0.50 & 68.34 & 89.42 & 0.54 & 66.00 & 0.89 & \textbf{0.97} & 31.50 & 0.00 & 0.72 & 60.01 & 0.00 & \underline{0.93} & 54.53 & 0.04 & 0.89 \\
 & Blended & 69.01 & 99.48 & 67.63 & 97.04 & 0.50 & 67.79 & 97.80 & 0.50 & 61.54 & 0.35 & \textbf{0.94} & 28.03 & 0.00 & 0.70 & 58.49 & 0.06 & \underline{0.92} & 42.89 & 2.03 & 0.80 \\
 & Wanet & 63.84 & 91.47 & 68.53 & 0.57 & 1.00 & 68.85 & 1.93 & \textbf{0.99} & 63.59 & 7.12 & 0.96 & 42.58 & 0.00 & 0.83 & 59.64 & 0.01 & \underline{0.97} & 57.04 & 0.90 & 0.94 \\
 \midrule[1.5pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% GTSRB 
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{6}{*}{\STAB{\rotatebox[origin=c]{90}{GTSRB}}} &
Attack & CA  & ASR  & CA  & ASR  & $\Gamma$ & CA  & ASR  &  $\Gamma$ & CA  & ASR  & $\Gamma$ & CA  &  ASR & $\Gamma$ & CA  & ASR  & $\Gamma$ & CA  & ASR  & $\Gamma$ \\
\midrule[0.5pt]
& Badnet & 96.61 & 83.86 & 97.97 & 51.80 & 0.69 & 97.76 & 57.30 & 0.66 & 96.85 & 0.00 & \textbf{1.00} & 92.03 & 0.00 & \underline{0.98} & 97.26 & 0.00 & \textbf{1.00} & 96.79 & 0.00 & \textbf{1.00} \\
 & Trojan & 98.17 & 100.0 & 98.70 & 100.0 & 0.50 & 96.93 & 0.17 & \textbf{0.99} & 93.45 & 2.70 & \underline{0.96} & 82.12 & 0.00 & 0.92 & 96.50 & 0.11 & \textbf{0.99} & 97.18 & 0.06 & \textbf{0.99} \\
 & Blended & 98.66 & 96.33 & 98.51 & 94.86 & 0.51 & 96.44 & 35.61 & 0.80 & 86.25 & 17.29 & 0.85 & 33.75 & 0.02 & 0.67 & 86.20 & 0.72 & \underline{0.93} & 89.94 & 3.67 & \textbf{0.94} \\
 & Wanet & 98.04 & 82.14 & 99.24 & 31.70 & 0.81 & 99.15 & 41.55 & 0.75 & 95.95 & 0.05 & \underline{0.99} & 79.90 & 29.31 & 0.73 & 97.14 & 0.33 & \underline{0.99} & 97.35 & 0.08 & \textbf{1.00} \\
 \midrule[1.5pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MEAN 
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{6}{*}{\STAB{\rotatebox[origin=c]{90}{MEAN}}} &
Attack & CA  & ASR  & CA  & ASR  & $\Gamma$ & CA  & ASR  &  $\Gamma$ & CA  & ASR  & $\Gamma$ & CA  &  ASR & $\Gamma$ & CA  & ASR  & $\Gamma$ & CA  & ASR  & $\Gamma$ \\
\midrule[0.5pt]
 & Badnet & 85.42 & 86.59 & 85.82 & 20.22 & 0.88 & 85.71 & 20.74 & 0.88 & 82.54 & 0.63 & \underline{0.98} & 76.48 & 0.00 & 0.94 & 83.74 & 0.28 & \textbf{0.99} & 83.60 & 0.58 & \underline{0.98} \\
 & Trojan & 87.06 & 100.0 & 86.98 & 99.77 & 0.50 & 86.11 & 63.12 & 0.68 & 74.43 & 4.67 & 0.91 & 64.02 & 2.84 & 0.84 & 80.04 & 2.29 & \textbf{0.95} & 76.02 & 0.93 & \underline{0.93} \\
 & Blended & 86.91 & 96.25 & 86.54 & 94.77 & 0.50 & 81.67 & 45.75 & 0.74 & 76.44 & 6.65 & \underline{0.91} & 50.69 & 0.73 & 0.78 & 76.93 & 1.88 & \textbf{0.93} & 73.45 & 2.76 & 0.90 \\
 & Signal & 92.90 & 89.04 & 93.51 & 83.87 & 0.53 & 81.79 & 6.81 & 0.90 & 89.23 & 18.03 & 0.88 & 80.71 & 4.51 & 0.91 & 87.18 & 0.31 & \textbf{0.97} & 89.94 & 7.51 & \underline{0.94} \\
 & Wanet & 83.95 & 90.40 & 87.05 & 16.88 & 0.90 & 87.11 & 18.12 & 0.89 & 83.48 & 2.82 & \textbf{0.98} & 69.52 & 10.98 & 0.84 & 81.77 & 0.90 & \textbf{0.98} & 79.58 & 0.51 & \underline{0.97} \\
%\bottomrule[1pt]
\bottomrule[1.2pt]
\end{tabular}
\label{tab:mainRes}
\end{table*}



    

==> sections/tables/mainRes_backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\caption{Results on the CIFAR10 dataset of four state-of-the-art backdoor defense methods alongside four configurations of our
method}
\footnotesize
\begin{tabular}{@{}l||l||cc||cc|cc|cc|cc||cc|cc||cc|cc@{}}
% HEADER
%\toprule[1.2pt]
%\toprule[1pt]
\hline
\multicolumn{1}{c}{\multirow{2}{*}{}} &
  \multicolumn{1}{c||}{\multirow{2}{*}{Method \faCaretRight}} &
  \multicolumn{2}{c||}{\multirow{2}{*}{Baseline}} &
  \multicolumn{2}{c|}{\multirow{2}{*}{FT}} &
  \multicolumn{2}{c|}{\multirow{2}{*}{NAD}} &
  \multicolumn{2}{c|}{\multirow{2}{*}{I-BAU}} &
  \multicolumn{2}{c||}{\multirow{2}{*}{MCL \cite{Yue2022ModelContrastiveLF}}} &
  \multicolumn{4}{c||}{Ours ($T_{pro}$)} &
  \multicolumn{4}{c}{Ours ($T_{syn}$)} \\
\cline{13-20}
% \cmidrule{13-20}
\multicolumn{1}{c}{} &
  \multicolumn{1}{c||}{} &
  \multicolumn{2}{c||}{} &
  \multicolumn{2}{c|}{} &
  \multicolumn{2}{c|}{} &
  \multicolumn{2}{c|}{} &
  \multicolumn{2}{c||}{} &
  \multicolumn{2}{c|}{$\delta$=0.75} &
  \multicolumn{2}{c||}{$\delta$ sch.} &
  \multicolumn{2}{c|}{$\delta$=0.75} &
  \multicolumn{2}{c}{$\delta$ sch.} \\
%\midrule[1pt]
% \multicolumn{20}{c}{}\\
%\midrule[1pt]
\hline\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CIFAR 10
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{6}{*}{\STAB{\rotatebox[origin=c]{90}{CIFAR10}}} &
  Attack \faCaretDown&
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ \\
\cline{2-20}
%  & Badnet & 92.34 & 88.93 & {\bf 92.66} & 8.43 & \underline{ 92.64} & 4.92 & 89.56 & 1.81 & 89.76 & \underline{ {\bf 0.01}} & 90.66 & 0.82 & 91.22 & 1.7 & \underline{ {\bf 92.8}} & {\bf 0.18} & 90.87 & \underline{ 0.7} \\ 
% & Trojan & 93 & 100 & \underline{ {\bf 93.3}} & 99.92 & {\bf 93.07} & 99.76 & 63.85 & 10.42 & 78.43 & 8.51 & 83.6 & {\bf 6.76} & 76.34 & \underline{ {\bf 2.68}} & 87.22 & 18.3 & \underline{ 89.92} & \underline{ 6.78} \\ 
% & Blended & 93.06 & 92.94 & \underline{ {\bf 93.47}} & 92.4 & 80.79 & 3.84 & 81.54 & {\bf 2.31} & \underline{ 90.28} & \underline{ {\bf 2.18}} & 86.11 & 4.87 & 87.51 & \underline{ 2.58} & 89.84 & 12.43 & {\bf 90.56} & 9.67 \\ 
% & Sig & 92.9 & 89.04 & \underline{ {\bf 93.51}} & 83.87 & 81.79 & 6.81 & \underline{ 89.23} & 18.03 & 80.71 & 4.51 & 87.18 & \underline{ {\bf 0.31}} & {\bf 89.94} & 7.51 &88.08 & {\bf 0.91} & 87.38 & \underline{ 3.6} \\ 
% & Wanet & 89.98 & 97.6 & \underline{ {\bf 93.39}} & 18.37 & {\bf 93.32} & 10.87 & \underline{ 90.9} & {\bf 1.3} & 86.08 & 3.64 & 88.54 & \underline{ 2.36} & 83.61 & \underline{ {\bf 0.61}} & 85.91 & 5.54 & 89.8 & 3.32 \\ 

& Badnet & 92.34 & 88.93 & {\bf 92.66} & 8.43 & \underline{ 92.64} & 4.92 & 89.56 & 1.81 & 89.76 & \underline{ {\bf 0.01}} & 90.66 & 0.82 & \underline{ {\bf 92.8}} & {\bf 0.18} & 91.22 & 1.7 & 90.87 & \underline{ 0.7} \\
& Trojan & 93 & 100 & \underline{ {\bf 93.3}} & 99.92 & {\bf 93.07} & 99.76 & 63.85 & 10.42 & 78.43 & 8.51 & 83.6 & {\bf 6.76} & 87.22 & 18.3 & 76.34 & \underline{ {\bf 2.68}} & \underline{ 89.92} & \underline{ 6.78} \\
& Blended & 93.06 & 92.94 & \underline{ {\bf 93.47}} & 92.4 & 80.79 & 3.84 & 81.54 & {\bf 2.31} & \underline{ 90.28} & \underline{ {\bf 2.18}} & 86.11 & 4.87 & 89.84 & 12.43 & 87.51 & \underline{ 2.58} & {\bf 90.56} & 9.67 \\
& Sig & 92.9 & 89.04 & \underline{ {\bf 93.51}} & 83.87 & 81.79 & 6.81 & \underline{ 89.23} & 18.03 & 80.71 & 4.51 & 87.18 & \underline{ {\bf 0.31}} & 88.08 & {\bf 0.91} & {\bf 89.94} & 7.51 & 87.38 & \underline{ 3.6} \\
& Wanet & 89.98 & 97.6 & \underline{ {\bf 93.39}} & 18.37 & {\bf 93.32} & 10.87 & \underline{ 90.9} & {\bf 1.3} & 86.08 & 3.64 & 88.54 & \underline{ 2.36} & 85.91 & 5.54 & 83.61 & \underline{ {\bf 0.61}} & 89.8 & 3.32 \\

%\midrule[1pt]
% \multicolumn{20}{c}{}\\
%\midrule[1pt]
\hline\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CIFAR 100
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{6}{*}{\STAB{\rotatebox[origin=c]{90}{CIFAR100}}} &
  Attack \faCaretDown &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ \\
\cline{2-20}

% & Badnet & 67.32 & 86.98 & \underline{ {\bf 66.82}} & 0.43 & {\bf 66.72} & 0.01 & 61.2 & 0.07 & 47.65 & \underline{ 0} & \underline{ 63.29} & 0.01 & 62.8 & 0.03 & 62.63 & \underline{ {\bf 0}} & 62.62 & {\bf 0} \\ 
% & Trojan & 70.02 & 100 & \underline{ {\bf 68.93}} & 99.4 & {\bf 68.34} & 89.42 & \underline{ 66} & 0.89 & 31.5 & \underline{ 0} & 60.01 & {\bf 0} & 54.53 & 0.04 & 60.01 & \underline{ {\bf 0}} & 59.34 & 0.01 \\ 
% & Blended & 69.01 & 99.48 & {\bf 67.63} & 97.04 & \underline{ {\bf 67.79}} & 97.8 & \underline{ 61.54} & 0.35 & 28.03 & \underline{ {\bf 0}} & 58.49 & {\bf 0.06} & 42.89 & 2.03 & 57.38 & \underline{ 0.16} & 58.3 & 44.16 \\ 
% & Wanet & 63.84 & 91.47 & {\bf 68.53} & 0.57 & \underline{ {\bf 68.85}} & 1.93 & \underline{ 63.59} & 7.12 & 42.58 & \underline{ {\bf 0}} & 59.64 & {\bf 0.01} & 57.04 & 0.9 & 60.33 & \underline{ 0.48} & 56.33 & 1.03 \\ 

& Badnet & 67.32 & 86.98 & \underline{ {\bf 66.82}} & 0.43 & {\bf 66.72} & 0.01 & 61.2 & 0.07 & 47.65 & \underline{ 0} & \underline{ 63.29} & 0.01 & 62.63 & \underline{ {\bf 0}} & 62.8 & 0.03 & 62.62 & {\bf 0} \\
& Trojan & 70.02 & 100 & \underline{ {\bf 68.93}} & 99.4 & {\bf 68.34} & 89.42 & \underline{ 66} & 0.89 & 31.5 & \underline{ 0} & 60.01 & {\bf 0} & 60.01 & \underline{ {\bf 0}} & 54.53 & 0.04 & 59.34 & 0.01 \\
& Blended & 69.01 & 99.48 & {\bf 67.63} & 97.04 & \underline{ {\bf 67.79}} & 97.8 & \underline{ 61.54} & 0.35 & 28.03 & \underline{ {\bf 0}} & 58.49 & {\bf 0.06} & 57.38 & \underline{ 0.16} & 42.89 & 2.03 & 58.3 & 44.16 \\
& Wanet & 63.84 & 91.47 & {\bf 68.53} & 0.57 & \underline{ {\bf 68.85}} & 1.93 & \underline{ 63.59} & 7.12 & 42.58 & \underline{ {\bf 0}} & 59.64 & {\bf 0.01} & 60.33 & \underline{ 0.48} & 57.04 & 0.9 & 56.33 & 1.03 \\

%\midrule[1pt]
% \Xhline{1.6pt}
% \multicolumn{20}{c}{}\\
% \Xhline{1.6pt}
%\midrule[1pt]
\hline\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% GTSRB
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{6}{*}{\STAB{\rotatebox[origin=c]{90}{GTSRB}}} &
  Attack \faCaretDown&
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ \\
\cline{2-20}


% & Badnet & 96.61 & 83.86 & \underline{ {\bf 97.97}} & 51.8 & {\bf 97.76} & 57.3 & 96.85 & 0 & 92.03 & \underline{ 0} & 97.26 & {\bf 0} & 96.79 & \underline{ {\bf 0}} & 97.45 & 0.04 & \underline{ 97.74} & 0.02 \\ 
% & Trojan & 98.17 & 100 & \underline{ {\bf 98.7}} & 100 & \underline{ 96.93} & 0.168 & 93.45 & 2.7 & 82.12 & \underline{ {\bf 0}} & 96.5 & 0.11 & {\bf 97.18} & \underline{ 0.06} & 95.8 & 1.25 & 96.27 & {\bf 0.02} \\ 
% & Blended & 98.66 & 96.33 & \underline{ {\bf 98.51}} & 94.86 & \underline{ 96.44} & 35.61 & 86.25 & 17.29 & 33.75 & {\bf 0.02} & 86.2 & \underline{ 0.72} & 89.94 & 3.67 & 95.24 & \underline{ {\bf 0}} & {\bf 96.73} & 3.08 \\ 
% & Wanet & 98.043 & 82.14 & \underline{ {\bf 99.24}} & 31.7 & {\bf 99.15} & 41.55 & 95.95 & {\bf 0.05} & 79.9 & 29.31 & 97.14 & \underline{ 0.33} & 97.35 & 0.08 & 97.78 & 0.5728 & \underline{ 98.08} & \underline{ {\bf 0.01}} \\ 

& Badnet & 96.61 & 83.86 & \underline{ {\bf 97.97}} & 51.8 & {\bf 97.76} & 57.3 & 96.85 & 0 & 92.03 & \underline{ 0} & 97.26 & {\bf 0} & 97.45 & 0.04 & 96.79 & \underline{ {\bf 0}} & \underline{ 97.74} & 0.02 \\
& Trojan & 98.17 & 100 & \underline{ {\bf 98.7}} & 100 & \underline{ 96.93} & 0.168 & 93.45 & 2.7 & 82.12 & \underline{ {\bf 0}} & 96.5 & 0.11 & 95.8 & 1.25 & {\bf 97.18} & \underline{ 0.06} & 96.27 & {\bf 0.02} \\
& Blended & 98.66 & 96.33 & \underline{ {\bf 98.51}} & 94.86 & \underline{ 96.44} & 35.61 & 86.25 & 17.29 & 33.75 & {\bf 0.02} & 86.2 & \underline{ 0.72} & 95.24 & \underline{ {\bf 0}} & 89.94 & 3.67 & {\bf 96.73} & 3.08 \\
& Wanet & 98.043 & 82.14 & \underline{ {\bf 99.24}} & 31.7 & {\bf 99.15} & 41.55 & 95.95 & {\bf 0.05} & 79.9 & 29.31 & 97.14 & \underline{ 0.33} & 97.78 & 0.5728 & 97.35 & 0.08 & \underline{ 98.08} & \underline{ {\bf 0.01}} \\

%\midrule[1pt]
% \Xhline{1.6pt}
% \multicolumn{20}{c}{}\\
% \Xhline{1.6pt}
%\midrule[1pt]
\hline\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MEAN
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{6}{*}{\STAB{\rotatebox[origin=c]{90}{MEAN}}} &
  Attack \faCaretDown&
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ &
  CA $\uparrow$ &
  ASR $\downarrow$ \\
\cline{2-20}

% & Badnet & 85.42 & 86.59 & \underline{ {\bf 85.82}} & 20.22 & {\bf 85.71} & 20.74 & 82.54 & 0.63 & 76.48 & \underline{ {\bf 0.00}} & \underline{ 83.74} & 0.28 & 83.60 & 0.58 & 84.29 & {\bf 0.07} & 83.74 & \underline{ 0.24} \\ 
% & Trojan & 87.06 & 100.00 & \underline{ {\bf 86.98}} & 99.77 & {\bf 86.11} & 63.12 & 74.43 & 4.67 & 64.02 & 2.84 & 80.04 & {\bf 2.29} & 76.02 & \underline{ {\bf 0.93}} & 81.01 & 6.52 & \underline{ 81.84} & \underline{ 2.27} \\
% & Blended & 86.91 & 96.25 & \underline{ {\bf 86.54}} & 94.77 & \underline{ 81.67} & 45.75 & 76.44 & 6.65 & 50.69 & \underline{ {\bf 0.73}} & 76.93 & {\bf 1.88} & 73.45 & \underline{ 2.76} & 80.82 & 4.20 & {\bf 81.86} & 18.97 \\ 
% & Sig & 92.90 & 89.04 & \underline{ {\bf 93.51}} & 83.87 & 81.79 & 6.81 & \underline{ 89.23} & 18.03 & 80.71 & 4.51 & 87.18 & \underline{ {\bf 0.31}} & {\bf 89.94} & 7.51 & 88.08 & {\bf 0.91} & 87.38 & \underline{ 3.60} \\ 
% & Wanet & 83.95 & 90.40 & {\bf 87.05} & 16.88 & \underline{ {\bf 87.11}} & 18.12 & \underline{ 83.48} & 2.82 & 69.52 & 10.98 & 81.77 & {\bf 0.90} & 79.58 & \underline{ {\bf 0.51}} & 81.34 & 2.20 & 81.40 & \underline{ 1.45} \\ 

& Badnet & 85.42 & 86.59 & \underline{ {\bf 85.82}} & 20.22 & {\bf 85.71} & 20.74 & 82.54 & 0.63 & 76.48 & \underline{ {\bf 0.00}} & \underline{ 83.74} & 0.28 & 84.29 & {\bf 0.07} & 83.60 & 0.58 & 83.74 & \underline{ 0.24} \\
& Trojan & 87.06 & 100.00 & \underline{ {\bf 86.98}} & 99.77 & {\bf 86.11} & 63.12 & 74.43 & 4.67 & 64.02 & 2.84 & 80.04 & {\bf 2.29} & 81.01 & 6.52 & 76.02 & \underline{ {\bf 0.93}} & \underline{ 81.84} & \underline{ 2.27} \\
& Blended & 86.91 & 96.25 & \underline{ {\bf 86.54}} & 94.77 & \underline{ 81.67} & 45.75 & 76.44 & 6.65 & 50.69 & \underline{ {\bf 0.73}} & 76.93 & {\bf 1.88} & 80.82 & 4.20 & 73.45 & \underline{ 2.76} & {\bf 81.86} & 18.97 \\
& Sig & 92.90 & 89.04 & \underline{ {\bf 93.51}} & 83.87 & 81.79 & 6.81 & \underline{ 89.23} & 18.03 & 80.71 & 4.51 & 87.18 & \underline{ {\bf 0.31}} & 88.08 & {\bf 0.91} & {\bf 89.94} & 7.51 & 87.38 & \underline{ 3.60} \\
& Wanet & 83.95 & 90.40 & {\bf 87.05} & 16.88 & \underline{ {\bf 87.11}} & 18.12 & \underline{ 83.48} & 2.82 & 69.52 & 10.98 & 81.77 & {\bf 0.90} & 81.34 & 2.20 & 79.58 & \underline{ {\bf 0.51}} & 81.40 & \underline{ 1.45} \\
\hline
%\bottomrule[1pt]
%\bottomrule[1.2pt]
\end{tabular}
\label{tab:mainRes}
\end{table*}



==> sections/tables/mainRes_dinov2.tex <==
\begin{table*}[t]
\caption{Ablation on distilling using dinoV2 with CIFAR10 dataset}
\label{tab:abl_distill}
\footnotesize
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{tabular}{l||cc||ccc|ccc||ccc|ccc}
\begin{tabular}{@{}L{12mm}||C{8mm}C{8mm}||C{8mm}C{8mm}C{8mm}|C{8mm}C{8mm}C{8mm}||C{8mm}C{8mm}C{8mm}|C{8mm}C{8mm}C{8mm}@{}}
\toprule[1.2pt]
%%%%%%%%%%%%%%%%%%%%%
Method \faCaretRight & \multicolumn{2}{c||}{Baseline} & \multicolumn{3}{c|}{PGBD $V^p$ with dinoV1} & \multicolumn{3}{c||}{PGBD $V^p$ with dinoV2} & \multicolumn{3}{c|}{PGBD $V^S$ with dinoV1} & \multicolumn{3}{c}{PGBD $V^S$ with dinoV2} \\
\midrule
Attack \faCaretDown & CA & ASR & CA & ASR & $\Gamma$ & CA & ASR & $\Gamma$ & CA & ASR & $\Gamma$ & CA & ASR & $\Gamma$  \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\specialrule{0.75pt}{1\jot}{1\jot}
%\hrule\hrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Badnet  & 92.34 & 88.93  & 90.66 & 0.82 & 0.99 & 91.22 & 1.70 & 0.98 & 87.44 & 0.11 & 0.97 & 88.86 & 0.92  & 0.98 \\
Trojan  & 93.00 & 100.00 & 83.60 & 6.76 & 0.92 & 76.34 & 2.68 & 0.90 & 87.41 & 0.76 & 0.97 & 89.03 & 1.56  & 0.97 \\
Blended & 93.06 & 92.94  & 86.11 & 4.87 & 0.94 & 87.51 & 2.58 & 0.96 & 89.38 & 3.12 & 0.96 & 88.41 & 11.10 & 0.92 \\
Sig     & 92.90 & 89.04  & 87.18 & 0.31 & 0.97 & 89.94 & 7.51 & 0.94 & 90.06 & 0.02 & 0.98 & 85.50 & 0.34  & 0.96 \\
Wanet   & 89.98 & 97.60  & 88.54 & 2.36 & 0.98 & 83.61 & 0.61 & 0.96 & 88.64 & 2.06 & 0.98 & 87.88 & 0.23  & 0.99 \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule[1.2pt]
\end{tabular}
\end{table*}

\begin{table*}[t]
\caption{Ablation on distilling using dinoV2 with CIFAR100 dataset}
\label{tab:abl_distill}
\footnotesize
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{tabular}{l||cc||ccc|ccc||ccc|ccc}
\begin{tabular}{@{}L{12mm}||C{8mm}C{8mm}||C{8mm}C{8mm}C{8mm}|C{8mm}C{8mm}C{8mm}||C{8mm}C{8mm}C{8mm}|C{8mm}C{8mm}C{8mm}@{}}
\toprule[1.2pt]
%%%%%%%%%%%%%%%%%%%%%
Method \faCaretRight & \multicolumn{2}{c||}{Baseline} & \multicolumn{3}{c|}{PGBD $V^p$ with dinoV1} & \multicolumn{3}{c||}{PGBD $V^p$ with dinoV2} & \multicolumn{3}{c|}{PGBD $V^S$ with dinoV1} & \multicolumn{3}{c}{PGBD $V^S$ with dinoV2} \\
\midrule
Attack \faCaretDown & CA & ASR & CA & ASR & $\Gamma$ & CA & ASR & $\Gamma$ & CA & ASR & $\Gamma$ & CA & ASR & $\Gamma$  \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\specialrule{0.75pt}{1\jot}{1\jot}
%\hrule\hrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Badnet  & 67.32 & 86.98  & 63.29 & 0.01 & 0.97 & 62.80 & 0.03 & 0.97 & 62.90 & 0.01 & 0.97 & 62.90 & 0.44  & 0.96 \\
Trojan  & 70.02 & 100.00 & 60.01 & 0.00 & 0.93 & 54.53 & 0.04 & 0.89 & 61.12 & 0.43 & 0.93 & 59.80 & 0.21  & 0.93 \\
Blended & 69.01 & 99.48  & 58.49 & 0.06 & 0.92 & 42.89 & 2.03 & 0.80 & 57.27 & 0.27 & 0.91 & 57.27 & 26.47 & 0.78 \\
Wanet   & 63.84 & 91.47  & 59.64 & 0.01 & 0.97 & 57.04 & 0.90 & 0.94 & 54.88 & 4.90 & 0.90 & 54.90 & 7.24  & 0.89 \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule[1.2pt]
\end{tabular}
\end{table*}


\begin{table*}[t]
\caption{Ablation on distilling using dinoV2 with GTSRB dataset}
\label{tab:abl_distill}
\footnotesize
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{tabular}{l||cc||ccc|ccc||ccc|ccc}
\begin{tabular}{@{}L{12mm}||C{8mm}C{8mm}||C{8mm}C{8mm}C{8mm}|C{8mm}C{8mm}C{8mm}||C{8mm}C{8mm}C{8mm}|C{8mm}C{8mm}C{8mm}@{}}
\toprule[1.2pt]
%%%%%%%%%%%%%%%%%%%%%
Method \faCaretRight & \multicolumn{2}{c||}{Baseline} & \multicolumn{3}{c|}{PGBD $V^p$ with dinoV1} & \multicolumn{3}{c||}{PGBD $V^p$ with dinoV2} & \multicolumn{3}{c|}{PGBD $V^S$ with dinoV1} & \multicolumn{3}{c}{PGBD $V^S$ with dinoV2} \\

\midrule
Attack \faCaretDown & CA & ASR & CA & ASR & $\Gamma$ & CA & ASR & $\Gamma$ & CA & ASR & $\Gamma$ & CA & ASR & $\Gamma$  \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\specialrule{0.75pt}{1\jot}{1\jot}
%\hrule\hrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Badnet  & 96.61 & 83.86  & 97.26 & 0.00 & 1.00 & 96.79 & 0.00 & 1.00 & 96.96 & 0.00 & 1.00 & 97.00 & 0.00 & 1.00 \\
Trojan  & 98.17 & 100.0 & 96.50 & 0.11 & 0.99 & 97.18 & 0.06 & 0.99 & 96.30 & 0.11 & 0.99 & 96.80 & 0.03 & 0.99 \\
Blended & 98.66 & 96.33  & 86.20 & 0.72 & 0.93 & 89.94 & 3.67 & 0.94 & 95.49 & 0.29 & 0.98 &       &      & 0.50 \\
Wanet   & 98.04 & 82.14  & 97.14 & 0.33 & 0.99 & 97.35 & 0.08 & 1.00 & 98.41 & 0.00 & 1.00 & 97.67 & 0.00 & 1.00 \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\bottomrule[1pt]
\bottomrule[1.2pt]
\end{tabular}
\end{table*}

==> sections/tables/related_works.tex <==
\begin{table}[t]
\centering
\caption{Defense strategies based on model life cycle. \\ (Access requirements legend: train/test data:\ding[1.25]{112}, validation data:\ding[1.25]{75}, model weight: (full) \ding[1.25]{108} (partial) \ding[1.25]{119} , training:\ding[1.25]{71}) }
\small
\begin{tabular}{@{}L{24mm}||R{60mm}@{}}
% \begin{tabular}{l||c}
% \toprule[1.2pt]
\toprule[1.5pt]
MODEL LIFECYLCE & DEFENSE STRATEGY \\
\midrule[1pt]
Before training & Training Data Sanitization \ding[1.25]{112}\ding[1.25]{71}  \cite{Taheri@2020,10.1007/978-3-030-13453-2_1,Tran2018SpectralSI,10.1016/j.cose.2021.102280,pmlr-v139-hayase21a} \\ 
\midrule[0.5pt]
During training & Differential Privacy \ding[1.25]{112}\ding[1.25]{71} \cite{li2021anti,DBLP:conf/iclr/ChenL0Z21} \\ 
\midrule[0.5pt] 
Post training & Model Inspection \ding[1.25]{112}\ding[1.25]{108} \cite{kolouri2020universal, xu2021detecting,chen2018detecting}, Model Sanitization \ding[1.25]{75} \ding[1.25]{119} \cite{Li2021NeuralAD,Yue2022ModelContrastiveLF, Zeng2021AdversarialUO}, Trigger Synthesis \ding[1.25]{112} \ding[1.25]{119} \cite{Wang2019NeuralCI, hu2021trigger,zhu2020gangsweep, Tao2022BetterTI}, Test Data Sanitization \ding[1.25]{112} \cite{chou2020sentinet,gao2019strip} \\
\bottomrule[1.5pt]
% \bottomrule[1.2pt]
\end{tabular}
\label{tab:realted_works}
\end{table}

==> sections/tables/semantic_results.tex <==
\begin{table}
\centering
% \footnotesize
\small
% \begin{tabular}{@{}l||cc|cc||cc@{}}
%\begin{tabular}{@{}l{16mm}||c{6mm}c{6mm}||c{6mm}c{6mm}c{6mm}||c{6mm}c{6mm}c{6mm}@{}}
%\begin{tabular}{L{16mm}|c{6mm}c{6mm}c{6mm}c{6mm}c{6mm}c{6mm}c{6mm}c{6mm}}
\begin{tabular}{l||cc|ccc|ccc}
% \hline 
\toprule[1.2pt]
%\toprule[1pt]
%Method \faCaretRight & \multicolumn{2}{c||}{Baseline} & 
 & \multicolumn{2}{c|}{\textbf{Baseline}} & \multicolumn{3}{c|}{\textbf{MCL}}      & \multicolumn{3}{c}{\textbf{PGBD ($V^p$)}} \\
%\hline %\midrule
Trigger & CA  & ASR  & CA  & ASR  & $\Gamma$ & CA  & ASR & $\Gamma$  \\
\midrule[1pt]
Sunglass  & 93.33 & 86.19 & 33.33 & 38.12 & 0.46 & 78.33 & 3.15 & \textbf{0.90} \\ 
%glasses & & & & & & & &\\ 
Tattoo & 78.4 & 72.1 & 40.38 & 2.38 & 0.74 & 86.53 & 2.4 & \textbf{0.98} \\
Mask & 69.23  & 96.66  &  21.1 & 9.6 & 0.6 & 63.46 & 3.33 &  \textbf{0.94}  \\
%\bottomrule[1pt]
% \hline 
\bottomrule[1.2pt]
\end{tabular}
\caption{Defense against semantic backdoor attacks. The Sunglass-based attack uses real images. Mask and tattoo-based attacks use synthetic triggers added using filters.}
\label{tab:semantic_res}
\end{table}
% \begin{table}[t ]
% \centering
% \caption{Defense results on our semantic attack for our method and MCL \TODO{Update table from sheets}}
% \footnotesize

% % \begin{tabular}{@{}l||cc|cc||cc@{}}
% \begin{tabular}{@{}L{24mm}||C{6mm}C{6mm}|C{6mm}C{6mm}||C{6mm}C{6mm}@{}}
% \toprule[1.2pt]
% \toprule[1pt]
% Method \faCaretRight & \multicolumn{2}{c|}{Baseline} & \multicolumn{2}{c||}{MCL \cite{Yue2022ModelContrastiveLF}}      & \multicolumn{2}{c}{PGBD ($V^p$)} \\
% \midrule
% Semantic Attack \faCaretDown & CA  & ASR  & CA  & ASR  & CA  & ASR  \\
% \midrule[1.5pt]
% Sunglasses & 93.33 & 86.19 & 33.33 & 38.12 & 71.67 & 4.97 \\ 
% Mask & 62.96  & 64.52   & 11.1  & 60.21   & 37.1  & 2.58  \\
% \bottomrule[1pt]
% \bottomrule[1.2pt]
% \end{tabular}
% \label{tab:semantic_res}
% \end{table}

==> sections/tables/tinyImagenet.tex <==
\begin{table*}
% \small
\footnotesize
\centering
%\begin{tabular}{@{}L{12mm}||C{8mm}C{8mm}|C{8mm}C{8mm}C{8mm}|C{8mm}C{8mm}C{8mm}|C{8mm}C{8mm}C{8mm}|C{8mm}C{8mm}C{8mm}||C{8mm}C{8mm}C{8mm}|C{8mm}C{8mm}C{8mm}@{}}
\begin{tabular}{l||cc||ccc||ccc|ccc}
\hline %\toprule[1.2pt]
%\toprule[1pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Method \faCaretRight & \multicolumn{2}{c||}{Baseline} & \multicolumn{6}{c||}{PGBD ($V^p$)} & \multicolumn{6}{c}{PGBD ($V^S$)}\\
%\midrule
%Distill \faCaretRight & \multicolumn{2}{c||}{$-$} & \multicolumn{3}{c|}{\CheckmarkBold} & \multicolumn{3}{c||}{\XSolidBrush} & \multicolumn{3}{c|}{\CheckmarkBold} & \multicolumn{3}{c}{\XSolidBrush} \\
% & & & \multicolumn{3}{c|}{PGBD ($V^p$)} With Distillation} & \multicolumn{3}{c||}{PGBD ($V^p$)} Without Distillation} & \multicolumn{3}{c|}{PGBD ($V^S$) With Distillation} & \multicolumn{3}{c}{PGBD ($V^S$) Without Distillation} \\
Method \faCaretRight & \multicolumn{2}{c||}{Baseline} & \multicolumn{3}{c||}{MCL} & \multicolumn{3}{c|}{PGBD $V^p$} & \multicolumn{3}{c}{PGBD $V^s$}  \\
\hline %\midrule
Attack \faCaretDown & CA & ASR & CA & ASR & $\Gamma$ & CA & ASR & $\Gamma$ & CA & ASR & $\Gamma$  \\
\hline %\midrule[1.5pt]

%%%%%%%%%%%%%%%%%%%%%%%%%%%
 % Attack & CA  & ASR  & CA  & ASR  & $\Gamma$ & CA  & ASR  &  $\Gamma$ & CA  & ASR  & $\Gamma$ & CA  &  ASR & $\Gamma$ & CA  & ASR  & $\Gamma$  \\
Badnet & 57.07 & 94.42 & 30.41 & 0 & 0.77 & 43.73 & 16.2 & 0.80 & 47.22 & 18.39 & 0.82 \\
Trojan & 59.93 & 98.56 & 20.39 & 0 & 0.67 & 41.22 & 22.05 & 0.73 & 37.12 & 20.64 & 0.70  \\
Blended & 57.04 & 95.59 & 32.3 & 16.58 & 0.70 & 42 & 14.99 & 0.79 & 40.73 & 17.2 & 0.77  \\
\hline %\bottomrule[1.2pt]
\end{tabular}
\caption{Quantitative comparison between MCL and four of our PGBD variants ($V^p$ and $V^s$) for tinyImagenet dataset.}
\label{tab:tinyImagenet}
\end{table*}
